A Quantitative Approach to Estimating Bias, Favouritism and Distortion in Scientific Journalism

While traditionally not considered part of the scientific method, science communication is increasingly playing a pivotal role in shaping scientific practice. Researchers are now frequently compelled to publicise their findings in response to institutional impact metrics and competitive grant environments. This shift underscores the growing influence of media narratives on both scientific priorities and public perception. In a current trend of personality-driven reporting, we examine patterns in science communication that may indicate biases of different types, towards topics and researchers. We focused and applied our methodology to a corpus of media coverage from three of the most prominent scientific media outlets: Wired, Quanta, and The New Scientist -- spanning the past 5 to 10 years. By mapping linguistic patterns, citation flows, and topical convergence, our objective was to quantify the dimensions and degree of bias that influence the credibility of scientific journalism. In doing so, we seek to illuminate the systemic features that shape science communication today and to interrogate their broader implications for epistemic integrity and public accountability in science. We present our results with anonymised journalist names but conclude that personality-driven media coverage distorts science and the practice of science flattening rather than expanding scientific coverage perception. Keywords : selective sourcing, bias, scientific journalism, Quanta, Wired, New Scientist, fairness, balance, neutrality, standard practices, distortion, personal promotion, communication, media outlets.

==> quanta_top_mentions_table_cleaned.tex <==
\textbf{Person} & \textbf{Mentions} \\
\hline
\textbf{Ben Brubaker} \\
%Turing & 40  \\
Peter Shor & 37  \\
Russell Impagliazzo & 36  \\
Bob Metcalfe & 30  \\
Marco Carmosino & 27  \\
\hline
\textbf{Charlie Wood} \\
%Richard Feynman & 89  \\
%Albert Einstein & 85  \\
Kin Fai Mak & 56  \\
%Stephen Hawking & 46  \\
Jie Shan & 43  \\
\hline
\textbf{Emily Singer} \\
Blair Hedges & 37  \\
Desai & 31  \\
Gerald Joyce & 25  \\
Nicholas Hud & 23  \\
Tobias & 23  \\
\hline
\textbf{Erica Klarreich} \\
Peter Scholze & 146  \\
Chris Maynard & 114  \\
Akshay Venkatesh & 70  \\
Mira Bhargava & 65  \\
Nikolaos Daskalakis & 61  \\
\hline
\textbf{John Pavlus} \\
Ellie Pavlick & 21  \\
Srinivasa Ramanujan & 21  \\
Yejin Choi & 20  \\
Pulkit Agrawal & 19  \\
Sam Bowman & 18  \\
\hline
\textbf{Jonathan O'Callaghan} \\
%James Clerk Maxwell & 11  \\
Beth Biller & 9  \\
Johansen & 9  \\
Merrill Sherman & 8  \\
Gonzalo Alonso-Álvarez & 7  \\
\hline
\textbf{Jordana Cepelewicz} \\
%Benoît Mandelbrot & 100  \\
Misha Lyubich & 87  \\
Huh & 57  \\
Terence Tao & 49  \\
Lucy Reading-Ikkanda & 43  \\
\hline
\textbf{Joshua Sokol} \\
Lisa Kaltenegger & 42  \\
Edward Lorenz & 38  \\
Gábor Domokos & 31  \\
Douglas Jerolmack & 23  \\
Daniel Rothman & 22  \\
\hline
\textbf{Kevin Hartnett} \\
June Huh & 86  \\
Robert Langlands & 76  \\
Lucy Reading-Ikkanda & 70  \\
Michael Freedman & 67  \\
%Erdos & 61  \\
\hline
\textbf{Leila Sloman} \\
Frank Ramsey & 36  \\
Zander Kelley & 28  \\
Raghu Meka & 27  \\
John McKay & 26  \\
Simkin & 25  \\
\hline
\textbf{Natalie Wolchover} \\
%Albert Einstein & 177  \\
Nima Arkani-Hamed & 104  \\
%Stephen Hawking & 104  \\
%Kurt Gödel & 75  \\
Wendy Freedman & 66  \\
\hline
\textbf{Philip Ball} \\
%Erwin Schrödinger & 42  \\
%Max Born & 37  \\
Michael Levin & 35  \\
Fernando Rosas & 22  \\
Robert Hazen & 22  \\
Lee Cronin &18\\
Giulio Tononi &16\\
\hline
\textbf{Pradeep Mutalik} \\
Srinivasa Ramanujan & 45  \\
Puzzle Columnist & 43  \\
Dan Pagefor & 24  \\
Rob Corlett & 20  \\
Sleeping Beauty & 19  \\
\hline
\textbf{Steve Nadis} \\
Shing-Tung Yau & 27  \\
Albert Einstein & 26  \\
Marcus Khuri & 25  \\
Cumrun Vafa & 21  \\
Eugenio Calabi & 21  \\
\hline
\textbf{Steven Strogatz} \\
%Steve Strogatz & 3279  \\
Alex Kontorovich & 337  \\
Priya Natarajan & 308  \\
Tadashi Tokieda & 241  \\
\hline
\textbf{Thomas Lin} \\
Maryna Viazovska & 65  \\
Subhash Khot & 59  \\
Artur Avila & 54  \\
Thomas Lin & 51  \\
Channa Comer & 46  \\
\hline
\textbf{Veronique Greenwood} \\
Carrie Partch & 50  \\
%Ratcliff & 34  \\
Carl Simpson & 25  \\
John Harte & 20  \\
Andreas Wagner & 16  \\
\hline
\textbf{Viviane Callier} \\
David Kingsley & 24  \\
Andrew Kern & 20  \\
Daniel Kronauer & 19  \\
Wesley McCutcheon & 17  \\
Daniel Rokhsar & 16  \\
\hline
\textbf{Yasemin Saplakoglu} \\
John Jumper & 47  \\
Ralph Nixon & 46  \\
Andreas Nieder & 43  \\
David Baker & 29  \\
John Moult & 29  \\
\hline
